Dataset Condensation for Recommendation

Training recommendation models on large datasets requires significant time and resources. It is desired to construct concise yet informative datasets for efficient training. Recent advances in dataset condensation show promise in addressing this problem by synthesizing small datasets. However, applying existing methods of dataset condensation to recommendation has limitations: (1) they fail to generate discrete user-item interactions, and (2) they could not preserve users' potential preferences. To address the limitations, we propose a lightweight condensation framework tailored for recommendation (DConRec), focusing on condensing user-item historical interaction sets. Specifically, we model the discrete user-item interactions via a probabilistic approach and design a pre-augmentation module to incorporate the potential preferences of users into the condensed datasets. While the substantial size of datasets leads to costly optimization, we propose a lightweight policy gradient estimation to accelerate the data synthesis. Experimental results on multiple real-world datasets have demonstrated the effectiveness and efficiency of our framework. Besides, we provide a theoretical analysis of the provable convergence of DConRec. Our implementation is available at: https://github.com/JiahaoWuGit/DConRec.

==> sections/merged-framework.tex <==
\begin{figure*}[htbp]
\centering
% \vskip -0.18in
{\includegraphics[width=0.7\linewidth]{{figures/merged-framework.pdf}}}
\vskip -0.05in
\caption{The process of dataset condensation for recommendation in a nutshell.}% (UC$^3$L).}
\vskip -0.08in
\label{fig:merged-condense-frameowork}
\end{figure*}

==> sections/sub-sections/alg-implementation-doscond.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
\caption{Implementation of DosCond}
\label{algo:doscond}
\REQUIRE a matrix $\mathbf{S}_{in}$, condensation ratio $r$.
\ENSURE projected matrix $\mathbf{S}_{out}$.
% \Procedure{Critical-Sample}{$\mathcal{D}$,$\boldsymbol{\theta}$}
    \STATE Firstly, calculate $s_{tmp_1}$ via:
    \[
    \mathbf{1}^T\left[\min\left(1,\max\left(0,\mathbf{S}_{in}-s_{tmp_1}\mathbf{1}\right)\right)\right]-r|\mathcal{D}|=0.
    \]
    \STATE Then, $s_{tmp_2}\leftarrow \max(0,s_{tmp_1})$.
    \STATE Finally, $\mathbf{S}_{out}\leftarrow \min\left(1,\max\left(0,\mathbf{S}_{in}-s_{tmp_2}\mathbf{1}\right)\right)$.
\STATE return $\mathbf{S}_{out}$
\end{algorithmic}
\end{algorithm}

==> sections/sub-sections/algorithms.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
\caption{Optimization algorithm of \red{OS-PGE}}
\label{algo:training}
\REQUIRE data pool $\mathcal{D}_{pool}$, validation dataset $\mathcal{D}_{val}$, a recommender model $\boldsymbol{\theta}$, condensation ratio $r$.
\ENSURE condensed dataset $\mathcal{D}_{s}$.
\STATE Initialize condensation probability $\bs{s}_{u,i}=r$%\bs{1}$
% \WHILE{Not Convergence}
% \STATE xxxx\\
% \STATE xxxx\\
\FOR{training iteration $t=1,2...T$}
    \STATE Sample selection matrix $\mathbf{M}$ based on the probability $\mathbf{S}$.\\
    \STATE Randomly initialize the model $\boldsymbol{\theta}_0$.\\
    \STATE Train the model for one epoch:
    \[
    \boldsymbol{\theta}_1 \leftarrow \boldsymbol{\theta}_0 - \nabla_{\boldsymbol{\theta}_0}\hat{\mathcal{L}}_{rec}(\boldsymbol{\theta}_0;\mathbf{M})
    \]
    % \STATE Sample a mini-batch interactions $\mathcal{B}$ from validation dataset $\mathcal{D}_{val}$.
    \STATE Update $\mathbf{S}$ based on Eq.~\ref{eq:one-step-gradient-s} based on validation dataset $\mathcal{D}_{val}$:
    \[
    \mathbf{S}^{t+1} \leftarrow \mathcal{P}_{\mathcal{C}}\left(\mathbf{S}^t-\eta \mathcal{L}_{\mathcal{D}_{val}}\left(\boldsymbol{\theta}_1(\mathbf{M})\right) \nabla_{\mathbf{S}^t} \ln p(\mathbf{M} \mid \mathbf{S}^t)\right)
    \]
    % \IF{$epoch_{idx}<N_{pre}$}
    % \STATE  xxxx\\
    % \ELSE
    %     \STATE xxxx 
    % \ENDIF
    % \STATE xxxxx \\
    % \STATE  xxxx   / xxxx\\
\ENDFOR
\STATE Sample $\mathbf{M}$ based on the probability $\mathbf{S}^{T+1}$.\\
\STATE Synthesize $\mathcal{D}_s$ based on selection matrix $\mathbf{M}$.
% \ENDWHILE
% \STATE $\textbf{z}_u$, $\textbf{z}_i=$  CF-Backbone($\mathcal{G}$, $\textbf{z}^{(0)}_u$, $\textbf{z}^{(0)}_i$); \textit{// Eq.~(\ref{eq:graph_prop})-(\ref{eq:layer_sum})}\\
\STATE return condensed dataset $\mathcal{D}_s$
\end{algorithmic}
\end{algorithm}




% \begin{algorithm}
% \begin{algorithmic}[1]
% \caption{Algorithm of \red{Critical Sampling, the algorithm need to be re-written}}
% \label{algo:critical-sampling}
% \REQUIRE original dataset $\mathcal{D}$, a proxy recommender model $\boldsymbol{\theta}$.%, pretrain epochs $N$.
% \ENSURE pseudo dataset $\mathcal{D}_{pseudo}$.
% % \Procedure{Critical-Sample}{$\mathcal{D}$,$\boldsymbol{\theta}$}
%     \STATE Initialization: $\mathcal{D}_{pseudo}\leftarrow\{\}$, $index\leftarrow 0$.%$epoch_{idx}\leftarrow 0$.
%         \FOR{$x$ in  \text{Dataloader}($\mathcal{D}$)} 
%             % \STATE \gray{//$\mathcal{B}=\{(u_1,pos_1,neg_1),...,(u_B,pos_B,neg_B)\}$}
%             % \STATE \brown{//$x=\{(u_1,pos_1),...,(u_B,pos_B)\}$}\\
%             % \STATE
%             % \STATE \gray{//(i) Model Update}
%             \STATE \gray{//$x=\{(u_1,pos_1),...,(u_B,pos_B)\}$}
%             \STATE Sample negative items for mini-batch $x$: 
%             \[
%             \mathcal{B}=\{(u_1,pos_1,neg_1),...,(u_B,pos_B,neg_B)\}
%             \]
%             \STATE Calculate the loss $\mathcal{L}(\mathcal{B};\theta)$.\\
%             % \STATE
%             % \STATE \gray{//(ii) Pseudo Data Generation}
%             % \IF{$epoch_{idx}>N$}
%             \STATE Obtain the negative item $neg_i$ with the largest loss in the mini-batch $\mathcal{B}$. 
%             \gray{//Denote $(u_{i},neg_{i})$ with $pair_{n}$}
%                 % \IF{$|\mathcal{D}_{pseudo}|>index$}
%                 %     \STATE In $\mathcal{D}_{pseudo}$, replace the $index$-th user-item pair with $pair_{n}$ if the preference score of $pair_{n}$ is larger than the $index$-th pair's. 
%                 % \ELSE
%             \STATE $\mathcal{D}_{pseudo}\leftarrow\mathcal{D}_{pseudo}\cup\{pair_{n}\}$
%                 % \ENDIF
%             % \ENDIF
%         \ENDFOR\\
%         $index\leftarrow index+1$.
% \STATE return $\mathcal{D}_{pseudo}$
% \end{algorithmic}
% \end{algorithm}




\begin{algorithm}
\begin{algorithmic}[1]
\caption{Algorithm of projection $\mathcal{P}_{\mathcal{C}}(\cdot)$}
\label{algo:projection}
\REQUIRE a matrix $\mathbf{S}_{in}$.
\ENSURE projected matrix $\mathbf{S}_{out}$.
% \Procedure{Critical-Sample}{$\mathcal{D}$,$\boldsymbol{\theta}$}
    \STATE Firstly, calculate $s_{tmp_1}$ via:
    \[
    \mathbf{1}^T\left[\min\left(1,\max\left(0,\mathbf{S}_{in}-s_{tmp_1}\mathbf{1}\right)\right)\right]-r|\mathcal{D}|=0.
    \]
    \STATE Then, $s_{tmp_2}\leftarrow \max(0,s_{tmp_1})$.
    \STATE Finally, $\mathbf{S}_{out}\leftarrow \min\left(1,\max\left(0,\mathbf{S}_{in}-s_{tmp_2}\mathbf{1}\right)\right)$.
\STATE return $\mathbf{S}_{out}$
\end{algorithmic}
\end{algorithm}
%the proof of this projection could be eliminated

==> sections/sub-sections/experiments/fig-ablation-study-module.tex <==
\begin{figure}[]
% \vskip -0.15in
\centering
% \subfigure[Ciao]{\label{fig:ciao-ablation-module}\includegraphics[width=0.498\columnwidth]{figures/experiments/ablation-study/Ciao-module-ablation.png}}
\subfigure[Gowalla]{\label{fig:gowalla-ablation-module}\includegraphics[width=0.495\columnwidth]{figures/experiments/ablation-study/Gowalla-merged-module-ablation.png}}
\subfigure[Dianping]{\label{fig:dianping-ablation-module}\includegraphics[width=0.495\columnwidth]{figures/experiments/ablation-study/Dianping-module-ablation.png}}
\vskip -0.15in
\caption{Ablation study on the effectiveness of the modules of the pseudo data and compensation for long-tailed users.}
%\red{you need to explain the signal of the variants and under what kind of condensation rate.}
\label{fig:ablation-study-module}
\vskip -0.05in
\end{figure}

==> sections/sub-sections/experiments/fig-pseudo-ratio-study-three-datasets.tex <==
\begin{figure}[]
\vskip -0.1in
\centering
\subfloat[Ciao-NDCG]{\label{fig:ciao-pseudo-ratio-ndcg}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Ciao-pseudo-data-ratio.png}}\hspace{0.025\columnwidth}
\subfloat[Ciao-Recall]{\label{fig:ciao-pseudo-ratio-ndcg}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Ciao-pseudo-data-ratio-recall.png}}
\vskip -0.08in

\subfloat[Gowalla-NDCG]{\label{fig:gowalla-pseudo-ratio-ndcg}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Gowalla-merged-pseudo-data-ratio.png}}\hspace{0.025\columnwidth}
\subfloat[Gowalla-Recall]{\label{fig:gowalla-pseudo-ratio-ndcg}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Gowalla-merged-pseudo-data-ratio-recall.png}}
\vskip -0.08in

\subfloat[Dianping-NDCG]{\label{fig:dianping-pseudo-ratio-ndcg}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Dianping-pseudo-data-ratio.png}}\hspace{0.025\columnwidth}
\subfloat[Dianping-Recall]{\label{fig:dianping-pseudo-ratio-ndcg}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Dianping-pseudo-data-ratio-recall.png}}
% \subfloat[Threshold Study]{\label{fig:ciao-threshold-study}\includegraphics[width=0.47\columnwidth]{figures/experiments/ciao-threshold-tail.png}}
% \subfigure[Dianping]{\label{fig:dianping-apseudo-ratio}\includegraphics[width=0.47\columnwidth]{figures/experiments/pseudo-data-study/Dianping-pseudo-data-ratio.png}}
\vskip -0.1in
\caption{Pseudo data ratio study while setting r to 0.25,0.5.}
\label{fig:pseudo-ratio-three-datasets}
\vskip -0.18in
\end{figure}

==> sections/sub-sections/experiments/fig-pseudo-ratio-study.tex <==
\begin{figure}[]
\vskip -0.1in
\centering
\subfloat[Pseudo Data Ratio Study]{\label{fig:ciao-pseudo-ratio}\includegraphics[width=0.495\columnwidth]{figures/experiments/pseudo-data-study/Ciao-pseudo-data-ratio.png}}
\subfloat[Threshold Study]{\label{fig:ciao-threshold-study}\includegraphics[width=0.495\columnwidth]{figures/experiments/ciao-threshold-tail.png}}
% \subfigure[Dianping]{\label{fig:dianping-apseudo-ratio}\includegraphics[width=0.66\columnwidth]{figures/experiments/pseudo-data-study/Dianping-pseudo-data-ratio.png}}
\vskip -0.15in
\caption{Parameter analysis while setting r to 0.25,0.5.}
\label{fig:pseudo-ratio}
\vskip -0.15in
\end{figure}

==> sections/sub-sections/experiments/fig-trainEfficiency-condenRatios.tex <==
\begin{figure}[t]
\vskip -0.05in
\centering
\subfloat[Pseudo Data Ratio Study]{\label{fig:subfig-trainingEfficiency}\includegraphics[width=0.495\columnwidth]{figures/experiments/training-efficiency/LightGCN-LightGCN-LightGCN-training-Efficiency.png}}
\subfloat[Threshold Study]{\label{fig:subfig-condenRatios}\includegraphics[width=0.495\columnwidth]{figures/experiments/different-condensed-ratios.png}}
% \subfigure[Dianping]{\label{fig:dianping-apseudo-ratio}\includegraphics[width=0.66\columnwidth]{figures/experiments/pseudo-data-study/Dianping-pseudo-data-ratio.png}}
\vskip -0.15in
\caption{Parameter analysis while setting r to 0.25,0.5.\red{remember to revise}}
\label{fig:trainEfficient-CondenRatios}
\vskip -0.05in
\end{figure}

==> sections/sub-sections/experiments/fig-training-efficiency.tex <==
\begin{figure}[htbp]
\vskip -0.05in
\centering
% \subfigure[With Model BPRMF]{\label{fig:ciao-pseudo-ratio}\includegraphics[width=0.495\columnwidth]{figures/experiments/training-efficiency/MF-MF-MF-trainingEfficiency.png}}
% \subfigure[With Model LightGCN]{
% \label{fig:xx}
\includegraphics[width=0.6\columnwidth]{figures/experiments/training-efficiency/LightGCN-LightGCN-LightGCN-training-Efficiency.png}
% }
\vskip -0.15in
\caption{Training efficiency on full dataset and dataset condensed by \ournameAbbr.}
\label{fig:training-efficiency}
\vskip -0.15in
\end{figure}

==> sections/sub-sections/experiments/plots/dianping-lightgcn.tex <==
\begin{tikzpicture}
\begin{axis}[    
    xlabel={Training Time (min)},
    ylabel={Recall@5},    
    ymin=0,    
    ymax=0.044,
    xmax=50,
    grid=both,
    grid style=dashed,
]

    \addplot[blue,line width=2pt] coordinates { %full 
        (0,0.0)
        (0.43,0.0168)
        (0.87,0.0163)
        (1.3,0.0167)
        (1.73,0.0167)
        (2.17,0.0167)
        (2.6,0.0167)
        (3.03,0.0168)
        (3.47,0.0169)
        (3.9,0.017)
        (4.33,0.0173)
        (4.77,0.0175)
        (5.2,0.0183)
        (5.63,0.0192)
        (6.06,0.0205)
        (6.5,0.0218)
        (6.93,0.0228)
        (7.36,0.0241)
        (7.8,0.0251)
        (8.23,0.0259)
        (8.66,0.0271)
        (9.1,0.0276)
        (9.53,0.0286)
        (9.96,0.0297)
        (10.4,0.0304)
        (10.83,0.0309)
        (11.26,0.0314)
        (11.7,0.0321)
        (12.13,0.0326)
        (12.56,0.0329)
        (13.0,0.0334)
        (13.43,0.0343)
        (13.86,0.0343)
        (14.3,0.0349)
        (14.73,0.0354)
        (15.16,0.0358)
        (15.6,0.0363)
        (16.03,0.0368)
        (16.46,0.0367)
        (16.9,0.0371)
        (17.33,0.0374)
        (17.76,0.0375)
        (18.19,0.038)
        (18.63,0.0378)
        (19.06,0.0381)
        (19.49,0.0385)
        (19.93,0.0384)
        (20.36,0.039)
        (20.79,0.0389)
        (21.23,0.0391)
        (21.66,0.0393)
        (22.09,0.0393)
        (22.53,0.0395)
        (22.96,0.0398)
        (23.39,0.0398)
        (23.83,0.04)
        (24.26,0.0401)
        (24.69,0.0403)
        (25.13,0.0403)
        (25.56,0.0408)
        (25.99,0.0406)
        (26.43,0.0412)
        (26.86,0.041)
        (27.29,0.041)
        (27.73,0.0411)
        (28.16,0.0413)
        (28.59,0.0413)
        (29.02,0.0412)
        (29.46,0.0413)
        (29.89,0.0415)
        (30.32,0.0416)
        (30.76,0.0419)
        (31.19,0.0423)
        (31.62,0.0421)
        (32.06,0.0423)
        (32.49,0.0426)
        (32.92,0.0425)
        (33.36,0.0423)
        (33.79,0.0425)
        (34.22,0.0424)
        (34.66,0.0423)
        (35.09,0.0428)
        (35.52,0.0427)
        (35.96,0.0427)
        (36.39,0.0433)
        (36.82,0.0433)
        (37.26,0.0437)
        (37.69,0.0436)
        (38.12,0.0435)
        (38.56,0.0435)
        (38.99,0.0436)
        (39.42,0.0435)
        (39.86,0.0432)
        (40.29,0.0436)
        (40.72,0.0435)
        (41.15,0.0435)
        (41.59,0.0437)
        (42.02,0.0437)
        (42.45,0.0436)
        (42.89,0.0437)
        (43.32,0.0436)
        (43.75,0.0437)
        (44.19,0.0436)
        (44.62,0.0434)
        (45.05,0.0435)
        (45.49,0.0435)
        (45.92,0.0432)
        (46.35,0.0434)
        (46.79,0.0435)
        (47.22,0.0435)
        (47.65,0.0433)
        (48.09,0.0432)
    };

    \addplot[orange,line width=2pt] coordinates {%DConRec
        (0,0.0)
        (0.05,0.0165)
        (0.11,0.0162)
        (0.16,0.0161)
        (0.22,0.0168)
        (0.27,0.0168)
        (0.33,0.0176)
        (0.38,0.0184)
        (0.43,0.0197)
        (0.49,0.0204)
        (0.54,0.0209)
        (0.6,0.0216)
        (0.65,0.0222)
        (0.71,0.0228)
        (0.76,0.0233)
        (0.81,0.0238)
        (0.87,0.024)
        (0.92,0.0243)
        (0.98,0.0248)
        (1.03,0.0249)
        (1.08,0.0254)
        (1.14,0.0255)
        (1.19,0.0256)
        (1.25,0.0259)
        (1.3,0.0261)
        (1.36,0.0266)
        (1.41,0.0268)
        (1.46,0.0268)
        (1.52,0.0273)
        (1.57,0.0274)
        (1.63,0.0275)
        (1.68,0.028)
        (1.74,0.0283)
        (1.79,0.0284)
        (1.84,0.0287)
        (1.9,0.0291)
        (1.95,0.0292)
        (2.01,0.0293)
        (2.06,0.0295)
        (2.12,0.0299)
        (2.17,0.03)
        (2.22,0.0302)
        (2.28,0.0304)
        (2.33,0.0307)
        (2.39,0.031)
        (2.44,0.0311)
        (2.49,0.0314)
        (2.55,0.0315)
        (2.6,0.0316)
        (2.66,0.0318)
        (2.71,0.032)
        (2.77,0.0322)
        (2.82,0.0324)
        (2.87,0.0323)
        (2.93,0.0324)
        (2.98,0.0324)
        (3.04,0.0325)
        (3.09,0.0327)
        (3.15,0.0324)
        (3.2,0.0326)
        (3.25,0.0328)
        (3.31,0.0329)
        (3.36,0.033)
        (3.42,0.0329)
        (3.47,0.0329)
        (3.53,0.0329)
        (3.58,0.0331)
        (3.63,0.0328)
        (3.69,0.033)
        (3.74,0.033)
        (3.8,0.033)
        (3.85,0.0332)
        (3.9,0.0332)
        (3.96,0.0333)
        (4.01,0.0332)
        (4.07,0.0332)
        (4.12,0.0334)
        (4.18,0.0333)
        (4.23,0.0333)
        (4.28,0.0336)
        (4.34,0.0333)
        (4.39,0.0334)
        (4.45,0.0336)
        (4.5,0.0337)
        (4.56,0.0336)
        (4.61,0.0338)
        (4.66,0.0335)
        (4.72,0.0336)
        (4.77,0.0337)
        (4.83,0.0337)
        (4.88,0.0337)
        (4.94,0.0338)
        (4.99,0.0337)
        (5.04,0.0338)
    };
    

\end{axis}
\end{tikzpicture}


==> sections/sub-sections/experiments/plots/dianping-mf.tex <==
\begin{tikzpicture}
\begin{axis}[    
    xlabel={Training Time (s)},
    ylabel={Recall@5},    
    ymin=0,    
    ymax=0.04,
    xmin=0,
    xmax=0.4,
    grid=both,
    grid style=dashed,
]


    \addplot[blue,line width=2pt] coordinates { %full 
        (0,0)
        (0.03,0.0082)
        (0.07,0.0137)
        (0.1,0.0149)
        (0.13,0.0161)
        (0.17,0.0167)
        (0.2,0.0169)
        (0.23,0.0169)
        (0.26,0.0166)
        (0.3,0.0165)
        (0.33,0.0168)
        (0.36,0.0168)
        (0.4,0.0168)
        (0.43,0.0169)
        (0.46,0.0168)
        (0.5,0.0175)
        (0.53,0.0179)
        (0.56,0.0175)
        (0.6,0.0178)
        (0.63,0.0174)
        (0.66,0.0176)
        (0.7,0.0181)
        (0.73,0.0182)
        (0.76,0.0186)
        (0.79,0.0184)
        (0.83,0.0186)
        (0.86,0.0188)
        (0.89,0.0186)
        (0.93,0.0192)
        (0.96,0.0196)
        (0.99,0.0201)
        (1.03,0.0202)
        (1.06,0.021)
        (1.09,0.0211)
        (1.13,0.0215)
        (1.16,0.0213)
        (1.19,0.0215)
        (1.23,0.0219)
        (1.26,0.022)
        (1.29,0.0224)
        (1.32,0.0225)
        (1.36,0.0224)
        (1.39,0.0226)
        (1.42,0.0229)
        (1.46,0.0234)
        (1.49,0.0239)
        (1.52,0.0243)
        (1.56,0.025)
        (1.59,0.0255)
        (1.62,0.026)
        (1.66,0.0259)
        (1.69,0.0263)
        (1.72,0.0262)
        (1.75,0.0264)
        (1.79,0.0267)
        (1.82,0.0264)
        (1.85,0.027)
        (1.89,0.0272)
        (1.92,0.0274)
        (1.95,0.0273)
        (1.99,0.0274)
        (2.02,0.0281)
        (2.05,0.028)
        (2.09,0.0282)
        (2.12,0.029)
        (2.15,0.0291)
        (2.19,0.0296)
        (2.22,0.0302)
        (2.25,0.0304)
        (2.28,0.0304)
        (2.32,0.0304)
        (2.35,0.0309)
        (2.38,0.0309)
        (2.42,0.0309)
        (2.45,0.0312)
        (2.48,0.0315)
        (2.52,0.0316)
        (2.55,0.0315)
        (2.58,0.0318)
        (2.62,0.0318)
        (2.65,0.0321)
        (2.68,0.0323)
        (2.72,0.0326)
        (2.75,0.0326)
        (2.78,0.0328)
        (2.81,0.0334)
        (2.85,0.0332)
        (2.88,0.0339)
        (2.91,0.0337)
        (2.95,0.0336)
        (2.98,0.0336)
        (3.01,0.0336)
        (3.05,0.0337)
        (3.08,0.0341)
        (3.11,0.0343)
        (3.15,0.0342)
        (3.18,0.0342)
        (3.21,0.0346)
        (3.25,0.0347)
        (3.28,0.0351)
        (3.31,0.0353)
        (3.34,0.0355)
        (3.38,0.0354)
        (3.41,0.0356)
        (3.44,0.036)
        (3.48,0.036)
        (3.51,0.036)
        (3.54,0.0359)
        (3.58,0.0362)
        (3.61,0.0362)
        (3.64,0.0361)
        (3.68,0.0362)
        (3.71,0.0366)
        (3.74,0.0364)
        (3.77,0.0364)
        (3.81,0.0366)
        (3.84,0.0366)
        (3.87,0.0369)
        (3.91,0.0368)
        (3.94,0.0369)
        (3.97,0.0369)
        (4.01,0.0372)
        (4.04,0.0372)
        (4.07,0.0373)
        (4.11,0.0373)
        (4.14,0.0372)
        (4.17,0.0373)
        (4.21,0.0372)
        (4.24,0.0375)
        (4.27,0.0378)
        (4.3,0.0377)
        (4.34,0.0377)
        (4.37,0.0376)
        (4.4,0.038)
        (4.44,0.0381)
        (4.47,0.0378)
        (4.5,0.0378)
        (4.54,0.0381)
        (4.57,0.0378)
        (4.6,0.038)
        (4.64,0.0378)
        (4.67,0.0379)
        (4.7,0.0379)
        (4.74,0.0379)
        (4.77,0.0383)
        (4.8,0.0382)
        (4.83,0.0382)
        (4.87,0.0382)
        (4.9,0.0378)
        (4.93,0.0379)
        (4.97,0.0378)
        (5.0,0.0378)
        (5.03,0.0377)
        (5.07,0.0379)
        (5.1,0.0377)
        (5.13,0.0376)
        (5.17,0.0379)
        (5.2,0.038)
        (5.23,0.0381)
        (5.26,0.0382)
        (5.3,0.0382)
        (5.33,0.0381)
        (5.36,0.0382)
        (5.4,0.0384)
        (5.43,0.0384)
        (5.46,0.0381)
        (5.5,0.0383)
        (5.53,0.0379)
        (5.56,0.038)
        (5.6,0.0379)
        (1.99,0.0082)
        (3.97,0.0137)
        (5.96,0.0149)
        (7.95,0.0161)
        (9.93,0.0167)
        (11.92,0.0169)
        (13.91,0.0169)
        (15.89,0.0166)
        (17.88,0.0165)
        (19.87,0.0168)
        (21.85,0.0168)
        (23.84,0.0168)
        (25.83,0.0169)
        (27.81,0.0168)
        (29.8,0.0175)
        (31.79,0.0179)
        (33.77,0.0175)
        (35.76,0.0178)
        (37.75,0.0174)
        (39.73,0.0176)
        (41.72,0.0181)
        (43.71,0.0182)
        (45.7,0.0186)
        (47.68,0.0184)
        (49.67,0.0186)
        (51.66,0.0188)
        (53.64,0.0186)
        (55.63,0.0192)
        (57.62,0.0196)
        (59.6,0.0201)
        (61.59,0.0202)
        (63.58,0.021)
        (65.56,0.0211)
        (67.55,0.0215)
        (69.54,0.0213)
        (71.52,0.0215)
        (73.51,0.0219)
        (75.5,0.022)
        (77.48,0.0224)
        (79.47,0.0225)
        (81.46,0.0224)
        (83.44,0.0226)
        (85.43,0.0229)
        (87.42,0.0234)
        (89.4,0.0239)
        (91.39,0.0243)
        (93.38,0.025)
        (95.36,0.0255)
        (97.35,0.026)
        (99.34,0.0259)
        (101.32,0.0263)
        (103.31,0.0262)
        (105.3,0.0264)
        (107.28,0.0267)
        (109.27,0.0264)
        (111.26,0.027)
        (113.24,0.0272)
        (115.23,0.0274)
        (117.22,0.0273)
        (119.2,0.0274)
        (121.19,0.0281)
        (123.18,0.028)
        (125.16,0.0282)
        (127.15,0.029)
        (129.14,0.0291)
        (131.13,0.0296)
        (133.11,0.0302)
        (135.1,0.0304)
        (137.09,0.0304)
        (139.07,0.0304)
        (141.06,0.0309)
        (143.05,0.0309)
        (145.03,0.0309)
        (147.02,0.0312)
        (149.01,0.0315)
        (150.99,0.0316)
        (152.98,0.0315)
        (154.97,0.0318)
        (156.95,0.0318)
        (158.94,0.0321)
        (160.93,0.0323)
        (162.91,0.0326)
        (164.9,0.0326)
        (166.89,0.0328)
        (168.87,0.0334)
        (170.86,0.0332)
        (172.85,0.0339)
        (174.83,0.0337)
        (176.82,0.0336)
        (178.81,0.0336)
        (180.79,0.0336)
        (182.78,0.0337)
        (184.77,0.0341)
        (186.75,0.0343)
        (188.74,0.0342)
        (190.73,0.0342)
        (192.71,0.0346)
        (194.7,0.0347)
        (196.69,0.0351)
        (198.67,0.0353)
        (200.66,0.0355)
        (202.65,0.0354)
        (204.63,0.0356)
        (206.62,0.036)
        (208.61,0.036)
        (210.6,0.036)
        (212.58,0.0359)
        (214.57,0.0362)
        (216.56,0.0362)
        (218.54,0.0361)
        (220.53,0.0362)
        (222.52,0.0366)
        (224.5,0.0364)
        (226.49,0.0364)
        (228.48,0.0366)
        (230.46,0.0366)
        (232.45,0.0369)
        (234.44,0.0368)
        (236.42,0.0369)
        (238.41,0.0369)
        (240.4,0.0372)
        (242.38,0.0372)
        (244.37,0.0373)
        (246.36,0.0373)
        (248.34,0.0372)
        (250.33,0.0373)
        (252.32,0.0372)
        (254.3,0.0375)
        (256.29,0.0378)
        (258.28,0.0377)
        (260.26,0.0377)
        (262.25,0.0376)
        (264.24,0.038)
        (266.22,0.0381)
        (268.21,0.0378)
        (270.2,0.0378)
        (272.18,0.0381)
        (274.17,0.0378)
        (276.16,0.038)
        (278.14,0.0378)
        (280.13,0.0379)
        (282.12,0.0379)
        (284.1,0.0379)
        (286.09,0.0383)
        (288.08,0.0382)
        (290.06,0.0382)
        (292.05,0.0382)
        (294.04,0.0378)
        (296.03,0.0379)
        (298.01,0.0378)
        (300.0,0.0378)
        (301.99,0.0377)
        (303.97,0.0379)
        (305.96,0.0377)
        (307.95,0.0376)
        (309.93,0.0379)
        (311.92,0.038)
        (313.91,0.0381)
        (315.89,0.0382)
        (317.88,0.0382)
        (319.87,0.0381)
        (321.85,0.0382)
        (323.84,0.0384)
        (325.83,0.0384)
        (327.81,0.0381)
        (329.8,0.0383)
        (331.79,0.0379)
        (333.77,0.038)
        (335.76,0.0379)
    };

    \addplot[orange,line width=2pt] coordinates {%DConRec
        (0,0)
        (0.02,0.0197)
        (0.04,0.0204)
        (0.07,0.0205)
        (0.09,0.021)
        (0.11,0.0214)
        (0.13,0.0215)
        (0.16,0.0218)
        (0.18,0.0223)
        (0.2,0.0224)
        (0.22,0.0225)
        (0.25,0.0223)
        (0.27,0.0224)
        (0.29,0.0228)
        (0.31,0.0229)
        (0.34,0.0228)
        (0.36,0.0231)
        (0.38,0.0238)
        (0.4,0.0244)
        (0.43,0.0247)
        (0.45,0.0249)
        (0.47,0.0253)
        (0.49,0.0255)
        (0.52,0.0257)
        (0.54,0.026)
        (0.56,0.0268)
        (0.58,0.0268)
        (0.61,0.027)
        (0.63,0.0277)
        (0.65,0.0283)
        (0.67,0.0284)
        (0.7,0.0287)
        (0.72,0.0292)
        (0.74,0.0293)
        (0.76,0.0293)
        (0.79,0.0295)
        (0.81,0.0299)
        (0.83,0.0301)
        (0.85,0.0302)
        (0.87,0.0304)
        (0.9,0.0308)
        (0.92,0.0312)
        (0.94,0.0315)
        (0.96,0.0313)
        (0.99,0.0317)
        (1.01,0.0319)
        (1.03,0.032)
        (1.05,0.0323)
        (1.08,0.0325)
        (1.1,0.0326)
        (1.12,0.0328)
        (1.14,0.0328)
        (1.17,0.0327)
        (1.19,0.0328)
        (1.21,0.0331)
        (1.23,0.0336)
        (1.26,0.0335)
        (1.28,0.0335)
        (1.3,0.0336)
        (1.32,0.0334)
        (1.35,0.0337)
        (1.37,0.0339)
        (1.39,0.0339)
        (1.41,0.0341)
        (1.44,0.0341)
        (1.46,0.0346)
        (1.48,0.0345)
        (1.5,0.0347)
        (1.53,0.0347)
        (1.55,0.0348)
        (1.57,0.0347)
        (1.59,0.0349)
        (1.62,0.0348)
        (1.64,0.0351)
        (1.66,0.035)
        (1.68,0.0351)
        (1.7,0.0351)
        (1.73,0.0353)
        (1.75,0.0351)
        (1.77,0.0355)
        (1.79,0.0354)
        (1.82,0.0355)
        (1.84,0.0355)
        (1.86,0.0358)
        (1.88,0.0358)
        (1.91,0.0357)
        (1.93,0.0362)
        (1.95,0.036)
        (1.97,0.0361)
        (2.0,0.0362)
        (2.02,0.0361)
        (2.04,0.0361)
        (2.06,0.0363)
        (2.09,0.0364)
        (2.11,0.0364)
        (2.13,0.0364)
        (2.15,0.0362)
        (2.18,0.0363)
        (2.2,0.0362)
        (2.22,0.0365)
        (1.35,0.0197)
        (2.69,0.0204)
        (4.04,0.0205)
        (5.38,0.021)
        (6.73,0.0214)
        (8.08,0.0215)
        (9.42,0.0218)
        (10.77,0.0223)
        (12.11,0.0224)
        (13.46,0.0225)
        (14.8,0.0223)
        (16.15,0.0224)
        (17.5,0.0228)
        (18.84,0.0229)
        (20.19,0.0228)
        (21.53,0.0231)
        (22.88,0.0238)
        (24.23,0.0244)
        (25.57,0.0247)
        (26.92,0.0249)
        (28.26,0.0253)
        (29.61,0.0255)
        (30.95,0.0257)
        (32.3,0.026)
        (33.65,0.0268)
        (34.99,0.0268)
        (36.34,0.027)
        (37.68,0.0277)
        (39.03,0.0283)
        (40.38,0.0284)
        (41.72,0.0287)
        (43.07,0.0292)
        (44.41,0.0293)
        (45.76,0.0293)
        (47.11,0.0295)
        (48.45,0.0299)
        (49.8,0.0301)
        (51.14,0.0302)
        (52.49,0.0304)
        (53.83,0.0308)
        (55.18,0.0312)
        (56.53,0.0315)
        (57.87,0.0313)
        (59.22,0.0317)
        (60.56,0.0319)
        (61.91,0.032)
        (63.26,0.0323)
        (64.6,0.0325)
        (65.95,0.0326)
        (67.29,0.0328)
        (68.64,0.0328)
        (69.98,0.0327)
        (71.33,0.0328)
        (72.68,0.0331)
        (74.02,0.0336)
        (75.37,0.0335)
        (76.71,0.0335)
        (78.06,0.0336)
        (79.41,0.0334)
        (80.75,0.0337)
        (82.1,0.0339)
        (83.44,0.0339)
        (84.79,0.0341)
        (86.13,0.0341)
        (87.48,0.0346)
        (88.83,0.0345)
        (90.17,0.0347)
        (91.52,0.0347)
        (92.86,0.0348)
        (94.21,0.0347)
        (95.56,0.0349)
        (96.9,0.0348)
        (98.25,0.0351)
        (99.59,0.035)
        (100.94,0.0351)
        (102.29,0.0351)
        (103.63,0.0353)
        (104.98,0.0351)
        (106.32,0.0355)
        (107.67,0.0354)
        (109.01,0.0355)
        (110.36,0.0355)
        (111.71,0.0358)
        (113.05,0.0358)
        (114.4,0.0357)
        (115.74,0.0362)
        (117.09,0.036)
        (118.44,0.0361)
        (119.78,0.0362)
        (121.13,0.0361)
        (122.47,0.0361)
        (123.82,0.0363)
        (125.16,0.0364)
        (126.51,0.0364)
        (127.86,0.0364)
        (129.2,0.0362)
        (130.55,0.0363)
        (131.89,0.0362)
        (133.24,0.0365)
    };
    

\end{axis}
\end{tikzpicture}


==> sections/sub-sections/experiments/plots/legend.tex <==
\begin{tikzpicture}
    \begin{customlegend}[
        legend columns=3,
        legend style={
            align=left,
            draw=none,
            column sep=2ex
        },
        legend entries={
            % \textsc{Original$_\text{NAML}$},
            % \textsc{Original$_\text{NRMS}$},
            % \textsc{Original$_\text{Fastformer}$},
            \textsc{DConRec},
            \textsc{Full Dataset},
            % \textsc{TF-DCon$_\text{Fastformer}$},
        }]
        % \addlegendimage{olive,mark=x,dotted,line legend}
        % \addlegendimage{orange,mark=x,dotted,line legend}
        % \addlegendimage{purple,mark=x,dotted,line legend}
        % \addlegendimage{blue,mark=x,solid,line legend}
        \addlegendimage{orange,solid,line legend}
        % \addlegendimage{orange,mark=x,solid,line legend}
        % \addlegendimage{purple,mark=x,solid,line legend}
        \addlegendimage{blue,solid,line legend}
        \end{customlegend}
\end{tikzpicture}


==> sections/sub-sections/experiments/plots/main.tex <==
% \begin{figure}
%     \centering
%     \setlength\tabcolsep{2pt}
    
%     \begin{tabular}{cc}
%     \multicolumn{2}{c}{
%         \resizebox{1.0\linewidth}{!}{
%             \input{sections/sub-sections/experiments/plots/legend}
%         }
%     } \\
%     % \begin{subfigure}{0.24\textwidth}
%         \resizebox{1.0\linewidth}{!}{
%             \input{sections/sub-sections/experiments/plots/dianping-mf}
%         }
%         % \caption{\label{fig:trend-mf}Training With BPRMF}
%     % \end{subfigure} %&
%     % \begin{subfigure}{0.24\textwidth}
%     %     \resizebox{1.0\linewidth}{!}{
%     %         \input{sections/sub-sections/experiments/plots/dianping-lightgcn}
%     %     }
%     %     \caption{\label{fig:trend-lightgcn}Training With LightGCN}
%     % \end{subfigure}
%     \end{tabular}

%     \vskip -0.05in
%     \caption{Training efficiency on full dataset and dataset condensed by DConRec.}
%     \label{fig:training-curve-on-datasets}
%     \vskip -0.15in
% \end{figure}




==> sections/sub-sections/experiments/tab-cross-architects-old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
% \vskip -0.05in
\caption{Generalization of DConRec. }
% \vskip -0.05in
\scalebox{1.0}{
\begin{tabular}{c|c|cccc}
\toprule%[1.2pt]
Backbone            & Test & R@5 & R@10 & N@5  & N@10  \\ \midrule
\multirow{4}{*}{LightGCN} & MF         & 0.0181  & 0.0289   & 0.0151 & 0.0186 \\
                          & NGCF       & 0.0178  & 0.0282   & 0.0153 & 0.0185  \\
                          & LightGCN   & 0.0188  & 0.0299   & 0.0163 & 0.0197  \\
                          & XSimGCL    & 0.0191  & 0.0298   & 0.0162 & 0.0195  \\ \midrule
\multirow{4}{*}{MF}       & MF         & 0.0180  & 0.0302   & 0.0163 & 0.0200  \\
                          & NGCF       & 0.0167  & 0.0282   & 0.0142 & 0.0179  \\
                          & LightGCN   & 0.0188  & 0.0300   & 0.0167 & 0.0201  \\
                          & XSimGCL    & 0.0192  & 0.0293   & 0.0163 & 0.0194  \\ \midrule
\multirow{4}{*}{NGCF}     & MF         & 0.0180  & 0.0289   & 0.0150 & 0.0184  \\
                          & NGCF       & 0.0177  & 0.0279   & 0.0156 & 0.0186 \\
                          & LightGCN   & 0.0187  & 0.0295   & 0.0162 & 0.0195  \\
                          & XSimGCL    & 0.0189  & 0.0299   & 0.0159 & 0.0193  \\ \midrule
\multirow{4}{*}{XSimGCL}  & MF         & 0.0180  & 0.0299   & 0.0151 & 0.0190  \\
                          & NGCF       & 0.0175  & 0.0277   & 0.0154 & 0.0185  \\
                          & LightGCN   & 0.0191  & 0.0299   & 0.0165 & 0.0197  \\
                          & XSimGCL    & 0.0187  & 0.0295   & 0.0160 & 0.0193  \\ \bottomrule%[1.2pt]
\end{tabular}
}
\label{tab:cross-architecture}
\vskip -0.1in
\end{table}

==> sections/sub-sections/experiments/tab-head-tail-compare-ciao.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Performance Comparison on Different User Groups.}
\vskip -0.12in
\scalebox{0.85}{\begin{tabular}{c|c|cccc}
\toprule[1.2pt]
Group                         & Methods   & Recall@5                                                       & Recall@10                                                      & NDCG@5                                                         & NDCG@10                                                        \\ \midrule
                              & SVP       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0305}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0468}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.1121}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0914}          \\
                              & GradMatch   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0273}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0420}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0954}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0794}          \\
                              & DConRec   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0343}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0547}}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.1245}}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.1041}}          \\
\multirow{-4}{*}{Head}  & Full Data & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0375}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0579}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.1418}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.1168}          \\ \midrule
                              & SVP       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0631}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.1002}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0414}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0534}          \\
                              & GradMatch   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0441}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0608}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0320}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0373}          \\
                              & DConRec   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0756}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.1150}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0524}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0650}} \\
\multirow{-4}{*}{Torso} & Full Data & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0853}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.1211}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0569}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0680}          \\ \midrule
                              & SVP       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0560}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0849}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0456}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0558}          \\
                              & GradMatch   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0389}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0608}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0327}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0406}          \\
                              & DConRec   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0623}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0946}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0519}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} \textbf{0.0634}} \\
\multirow{-4}{*}{Tail}  & Full Data & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0682}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.1024}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0577}          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{1F1F1F} 0.0697}          \\ \bottomrule[1.2pt]
\end{tabular}}
\label{tab:head-tail-performance}
\vskip -0.05in
\end{table}

==> sections/sub-sections/experiments/tab-overall-compare-05AND025.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
% \vskip -0.15in
\centering
\caption{Performance comparison compared to baselines. \textit{C. R.} denotes the condensation ratio of datasets, \textit{Full Dataset} indicates the performance with original datasets and \textit{Com. to Full} denotes the performance achieved by our proposed methods when compared to performance with original datasets.}% $\Delta$
\scalebox{1.0}{
\begin{tabular}{c|c|c|ccc|cc|c|c}
\toprule[1.2pt]
\multirow{2}{*}{Dataset}  & \multirow{2}{*}{C. R.} & \multicolumn{1}{c|}{\multirow{2}{*}{Metrics}} & \multicolumn{3}{c|}{Sampling-Based} & \multicolumn{2}{c|}{\red{Synthesizing-Based}} & \multirow{2}{*}{Com. to Full} & \multicolumn{1}{c}{\multirow{2}{*}{Full Dataset}} \\
                          &                              & \multicolumn{1}{c|}{}                         & Random    & Majority    & SVP       & DosCond        & \textit{DConRec}       &                               & \multicolumn{1}{c}{}                              \\ \midrule[1.0pt]
\multirow{8}{*}{Ciao}     & \multirow{4}{*}{0.25}        & Recall@5                                      & 0.0062    & 0.0115      & 0.0164    & 0.0081         & \textbf{0.0180}        & 91.24\%                       & 0.0197                                            \\
                          &                              & Recall@10                                     & 0.0092    & 0.0180      & 0.0289    & 0.0124         & \textbf{0.0302}        & 96.71\%                       & 0.0312                                            \\
                          &                              & NDCG@5                                        & 0.0071    & 0.0097      & 0.0148    & 0.0080         & \textbf{0.0163}        & 91.57\%                       & 0.0178                                            \\
                          &                              & NDCG@10                                       & 0.0076    & 0.0117      & 0.0187    & 0.0092         & \textbf{0.0200}        & 94.34\%                       & 0.0212                                            \\ \cmidrule{2-10} 
                          & \multirow{4}{*}{0.5}         & Recall@5                                      & 0.0106    & 0.0169      & 0.0170    & 0.0158         & \textbf{0.0179}        & 90.74\%                       & 0.0197                                            \\
                          &                              & Recall@10                                     & 0.0179    & 0.0280      & 0.0269    & 0.0236         & \textbf{0.0309}        & 99.04\%                       & 0.0312                                            \\
                          &                              & NDCG@5                                        & 0.0106    & 0.0130      & 0.0154    & 0.0150         & \textbf{0.0168}        & 94.52\%                       & 0.0178                                            \\
                          &                              & NDCG@10                                       & 0.0126    & 0.0170      & 0.0184    & 0.0171         & \textbf{0.0198}        & 93.16\%                       & 0.0212                                            \\ \midrule[1.0pt]
\multirow{8}{*}{Gowalla}  & \multirow{4}{*}{0.25}        & Recall@5                                      & 0.0300    & 0.0461      & 0.0540    & 0.0362         & \textbf{0.0622}        & 91.61\%                       & 0.0679                                            \\
                          &                              & Recall@10                                     & 0.0457    & 0.0667      & 0.0836    & 0.0548         & \textbf{0.0930}        & 91.63\%                       & 0.1015                                            \\
                          &                              & NDCG@5                                        & 0.0277    & 0.0336      & 0.0474    & 0.0337         & \textbf{0.0558}        & 90.11\%                       & 0.0619                                            \\
                          &                              & NDCG@10                                       & 0.0327    & 0.0404      & 0.0567    & 0.0394         & \textbf{0.0651}        & 90.42\%                       & 0.0720                                            \\ \cmidrule{2-10} 
                          & \multirow{4}{*}{0.5}         & Recall@5                                      & 0.0530    & 0.0626      & 0.0580    & 0.0622         & \textbf{0.0670}        & 98.64\%                       & 0.0679                                            \\
                          &                              & Recall@10                                     & 0.0811    & 0.0923      & 0.0880    & 0.0919         & \textbf{0.0996}        & 98.13\%                       & 0.1015                                            \\
                          &                              & NDCG@5                                        & 0.0488    & 0.0484      & 0.0518    & 0.0574         & \textbf{0.0604}        & 97.62\%                       & 0.0619                                            \\
                          &                              & NDCG@10                                       & 0.0574    & 0.0590      & 0.0612    & 0.0664         & \textbf{0.0703}        & 97.64\%                       & 0.0720                                            \\ \midrule[1.0pt]
\multirow{8}{*}{Dianping} & \multirow{4}{*}{0.25}        & Recall@5                                      & 0.0091    & 0.0134      & 0.0314    & 0.0115         & \textbf{0.0370}        & 99.26\%                       & 0.0373                                            \\
                          &                              & Recall@10                                     & 0.0169    & 0.0236      & 0.0523    & 0.0200         & \textbf{0.0614}        & 99.80\%                       & 0.0615                                            \\
                          &                              & NDCG@5                                        & 0.0065    & 0.0086      & 0.0216    & 0.0082         & \textbf{0.0259}        & 97.56\%                       & 0.0266                                            \\
                          &                              & NDCG@10                                       & 0.0091    & 0.0120      & 0.0285    & 0.0111         & \textbf{0.0340}        & 98.19\%                       & 0.0346                                            \\ \cmidrule{2-10} 
                          & \multirow{4}{*}{0.5}         & Recall@5                                      & 0.0134    & 0.0276      & 0.0301    & 0.0207         & \textbf{0.0389}        & 104.22\%                      & 0.0373                                            \\
                          &                              & Recall@10                                     & 0.0239    & 0.0468      & 0.0516    & 0.0347         & \textbf{0.0638}        & 103.74\%                      & 0.0615                                            \\
                          &                              & NDCG@5                                        & 0.0094    & 0.0179      & 0.0211    & 0.0148         & \textbf{0.0274}        & 102.82\%                      & 0.0266                                            \\
                          &                              & NDCG@10                                       & 0.0129    & 0.0242      & 0.0282    & 0.0195         & \textbf{0.0356}        & 102.75\%                      & 0.0346                                            \\ \bottomrule[1.2pt]
\end{tabular}
}
\label{tab:overall-com}
% \vskip -0.07in
\end{table*}

==> sections/sub-sections/experiments/tab-overall-compare025-original.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
% \vskip -0.15in
\centering
\caption{Performance comparison compared to baselines. \textit{Full Dataset} indicates the performance with original datasets and \textit{Quality} denotes the performance achieved by our proposed methods when compared to performance with original datasets.\red{add several methods here.}}% $\Delta$
\vskip -0.1in
\scalebox{1.0}{
\begin{tabular}{c|c|ccc|cc|c|c}
\toprule[1.2pt]
\multirow{2}{*}{Dataset}  &  \multicolumn{1}{c|}{\multirow{2}{*}{Metrics}} & \multicolumn{3}{c|}{Selection-based} & \multicolumn{2}{c|}{{Condensation-based}} & \multirow{2}{*}{Quality} & \multicolumn{1}{c}{\multirow{2}{*}{Full Dataset}} \\
                          &  \multicolumn{1}{c|}{}                         & Random    & Majority    & SVP       & GradMatch        & \textit{DConRec}       &                               & \multicolumn{1}{c}{}                              \\ \midrule[1.0pt]
\multirow{4}{*}{Ciao}        & Recall@5                                      & 0.0062    & 0.0115      & 0.0164    & 0.0081         & \textbf{0.0180}        & 91.24\%                       & 0.0197                                            \\
                          &Recall@10                                     & 0.0092    & 0.0180      & 0.0289    & 0.0124         & \textbf{0.0302}        & 96.71\%                       & 0.0312                                            \\
                          & NDCG@5                                        & 0.0071    & 0.0097      & 0.0148    & 0.0080         & \textbf{0.0163}        & 91.57\%                       & 0.0178                                            \\
                          &NDCG@10                                       & 0.0076    & 0.0117      & 0.0187    & 0.0092         & \textbf{0.0200}        & 94.34\%                       & 0.0212                                            \\ %\cmidrule{2-10} 
                          % & \multirow{4}{*}{0.5}         & Recall@5                                      & 0.0106    & 0.0169      & 0.0170    & 0.0158         & \textbf{0.0179}        & 90.74\%                       & 0.0197                                            \\
                          % &                              & Recall@10                                     & 0.0179    & 0.0280      & 0.0269    & 0.0236         & \textbf{0.0309}        & 99.04\%                       & 0.0312                                            \\
                          % &                              & NDCG@5                                        & 0.0106    & 0.0130      & 0.0154    & 0.0150         & \textbf{0.0168}        & 94.52\%                       & 0.0178                                            \\
                          % &                              & NDCG@10                                       & 0.0126    & 0.0170      & 0.0184    & 0.0171         & \textbf{0.0198}        & 93.16\%                       & 0.0212                                            \\ 
                          \midrule[1.0pt]
\multirow{4}{*}{Gowalla}       & Recall@5                                      & 0.0300    & 0.0461      & 0.0540    & 0.0362         & \textbf{0.0622}        & 91.61\%                       & 0.0679                                            \\
                          & Recall@10                                     & 0.0457    & 0.0667      & 0.0836    & 0.0548         & \textbf{0.0930}        & 91.63\%                       & 0.1015                                            \\
                          & NDCG@5                                        & 0.0277    & 0.0336      & 0.0474    & 0.0337         & \textbf{0.0558}        & 90.11\%                       & 0.0619                                            \\
                          & NDCG@10                                       & 0.0327    & 0.0404      & 0.0567    & 0.0394         & \textbf{0.0651}        & 90.42\%                       & 0.0720                                            \\ %\cmidrule{2-10} 
                          % & \multirow{4}{*}{0.5}         & Recall@5                                      & 0.0530    & 0.0626      & 0.0580    & 0.0622         & \textbf{0.0670}        & 98.64\%                       & 0.0679                                            \\
                          % &                              & Recall@10                                     & 0.0811    & 0.0923      & 0.0880    & 0.0919         & \textbf{0.0996}        & 98.13\%                       & 0.1015                                            \\
                          % &                              & NDCG@5                                        & 0.0488    & 0.0484      & 0.0518    & 0.0574         & \textbf{0.0604}        & 97.62\%                       & 0.0619                                            \\
                          % &                              & NDCG@10                                       & 0.0574    & 0.0590      & 0.0612    & 0.0664         & \textbf{0.0703}        & 97.64\%                       & 0.0720                                            \\ 
                          \midrule[1.0pt]
\multirow{4}{*}{Dianping} & Recall@5                                      & 0.0091    & 0.0134      & 0.0314    & 0.0115         & \textbf{0.0370}        & 99.26\%                       & 0.0373                                            \\
                          & Recall@10                                     & 0.0169    & 0.0236      & 0.0523    & 0.0200         & \textbf{0.0614}        & 99.80\%                       & 0.0615                                            \\
                          & NDCG@5                                        & 0.0065    & 0.0086      & 0.0216    & 0.0082         & \textbf{0.0259}        & 97.56\%                       & 0.0266                                            \\
                          & NDCG@10                                       & 0.0091    & 0.0120      & 0.0285    & 0.0111         & \textbf{0.0340}        & 98.19\%                       & 0.0346                                            \\ %\cmidrule{2-10} 
                          % & \multirow{4}{*}{0.5}         & Recall@5                                      & 0.0134    & 0.0276      & 0.0301    & 0.0207         & \textbf{0.0389}        & 104.22\%                      & 0.0373                                            \\
                          % &                              & Recall@10                                     & 0.0239    & 0.0468      & 0.0516    & 0.0347         & \textbf{0.0638}        & 103.74\%                      & 0.0615                                            \\
                          % &                              & NDCG@5                                        & 0.0094    & 0.0179      & 0.0211    & 0.0148         & \textbf{0.0274}        & 102.82\%                      & 0.0266                                            \\
                          % &                              & NDCG@10                                       & 0.0129    & 0.0242      & 0.0282    & 0.0195         & \textbf{0.0356}        & 102.75\%                      & 0.0346                                            \\ 
                          \bottomrule[1.2pt]
\end{tabular}
}
\label{tab:overall-com}
% \vskip -0.05in
\end{table*}

==> sections/sub-sections/experiments/tab-proxy-models-ciao.tex <==
\begin{table}[htbp]
% \vskip -0.1in
\caption{Effects of Different Architectures of Poxy Model.}
\vskip -0.1in
\scalebox{0.9}{
\begin{tabular}{c|cccc}
\toprule[1.2pt]
Proxy Model & Recall@5 & Recall@10 & NDCG@5   & NDCG@10  \\ \midrule
MF          & 0.01800    & 0.03020    & 0.01630   & 0.02000     \\ %\midrule
NGCF        & 0.01753 & 0.02930    & 0.01478 & 0.01863 \\ %\midrule
LightGCN    & 0.01928 & 0.02968  & 0.01663 & 0.01968 \\ %\midrule
XSimGCL     & 0.01933 & 0.03280    & 0.01668 & 0.02083 \\ \bottomrule[1.2pt]
\end{tabular}
}
\label{tab:proxy-model-study}
\vskip -0.1in

\end{table}

==> sections/sub-sections/fig-intro-dc.tex <==
\begin{figure}[]
% \vskip -0.1in
\centering
% \vskip -0.18in
% {\includegraphics[width=1.0\linewidth]{{figures/intro-dd-compar2.pdf}}}
{\includegraphics[width=0.85\linewidth]{{figures/DC-intro.pdf}}}
\vskip -0.1in
\caption{An overview of dataset condensation.\red{delete}}
\vskip -0.2in
\label{fig:intro-dc}
\end{figure}



==> sections/sub-sections/fig-os-pge.tex <==
\begin{figure}[]
\centering
% \vskip -0.18in
{\includegraphics[width=1.0\linewidth]{{figures/pdc-framework-19.pdf}}}
\vskip -0.05in
\caption{The process of dataset condensation for recommendation in a nutshell.}% (UC$^3$L).}
\vskip -0.15in
\label{fig:condense-frameowork}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}


==> sections/sub-sections/fig-pseudo-data.tex <==
% \begin{figure*}[htbp]
% \centering
% % \vskip -0.18in
% {\includegraphics[width=0.7\linewidth]{{figures/data-pool-2.pdf}}}
% \vskip -0.05in
% \caption{Generation of Data Pool.}% (UC$^3$L).}
% \vskip -0.08in
% \label{fig:pseudo-data-generation}
% \end{figure*}

\begin{figure}[]%[htbp]
\centering
% \vskip -0.18in
{\includegraphics[width=0.6\linewidth]{{figures/data-pool-gene7.pdf}}}
\vskip -0.05in
\caption{Generate data pool via pre-augmentation.}% (UC$^3$L).}
\vskip -0.15in
\label{fig:pseudo-data-generation}
\end{figure}


==> sections/sub-sections/figures.tex <==
\begin{figure*}[]%[htbp]
\centering
% \vskip -0.18in
{\includegraphics[width=0.7\linewidth]{{figures/data-pool-2.pdf}}}
\vskip -0.05in
\caption{Generation of Data Pool.}% (UC$^3$L).}
\vskip -0.08in
\label{fig:pseudo-data-generation}
\end{figure*}

\begin{figure*}[]%[htbp]
\centering
% \vskip -0.18in
{\includegraphics[width=0.7\linewidth]{{figures/pdc-framework-2.pdf}}}
\vskip -0.05in
\caption{The process of dataset condensation for recommendation in a nutshell.}% (UC$^3$L).}
\vskip -0.08in
\label{fig:condense-frameowork}
\end{figure*}
